SeReNe: Sensitivity based Regularization of Neurons for Structured Sparsity in Neural Networks

Deep neural networks include millions of learnable parameters, making their deployment over resource-constrained devices problematic. SeReNe (Sensitivity-based Regularization of Neurons) is a method for learning sparse topologies with a structure, exploiting neural sensitivity as a regularizer. We define the sensitivity of a neuron as the variation of the network output with respect to the variation of the activity of the neuron. The lower the sensitivity of a neuron, the less the network output is perturbed if the neuron output changes. By including the neuron sensitivity in the cost function as a regularization term, we areable to prune neurons with low sensitivity. As entire neurons are pruned rather then single parameters, practical network footprint reduction becomes possible. Our experimental results on multiple network architectures and datasets yield competitive compression ratios with respect to state-of-the-art references.

==> 2_related_old.tex <==
\section{Related work}
\label{sec:related}

%\textbf{XXX AF: Qui dobbiamo spiegare che questa é una overview esclusivamente dei metodi di training di rete sparse, che é l'oggetto della nostra ricerca, motivo per cui il lettore non troverà nulla su quantizzazione, filtri separabili, etc.

%L ideale sarebbe organizzare le referenze per classe o tipologia, in ogni caso dando una visione schematica dello stato dell arte in materia.
%Per ogni referenza che citiamo, sarebe ottimo concludere con un paio di rifge che spieghino quali siano i limiti di tale metodo.
%}

Approaches towards compact neural networks representations can be categorized in three major groups: altering the network structure, quantizing the parameters and pruning weights. % \added{and knowledge distillation}.
In this section, we review works based on a pruning approach that are most relevant to our work.
%, that fall in the last class, i.e. compression of artificial neural network networks via pruning.

% In the remainder of this section we give a summary of the main techniques and their drawbacks. A more in depth analysis on the topic has been published by Gale \textit{et al}. \cite{gale:state}.

% An approach requires an $L_0$ regularization to prune the network parameters during training (e.g. Louizos \textit{et al}. \cite{louizos:sparse_l0}). This technique penalizes non-zero value of a parameters vector, promoting sparse solutions; however, it requires to solve highly complex optimization problem as well as a lack of flexibility. 

% In recent years techniquest based on the notion of the dropout proposed by \cite{srivastava:dropout} have been employed. Dropout is a regularization method for deep neural networks which add multiplicative random noise to the input of each layer of the neural network during training. In this way parameters are less likely to overfit the training data.

% Kingma \textit{et al.} \cite{kingma:var_dropout} show that dropout can be seen as a special
% case of Bayesian regularization while Molachanov \textit{et al.} \cite{molchanov:var_dropout} propose an extension to Variational Dropout in the case when each weight of a network has its individual dropout rate.

% Another kind of approach is to define the importance of each connection and later remove parameters deemed unnecessary. For example, Han \textit{et al} \cite{han:learning} define said importance minimizing a target loss function. Another variation was proposed by Tartaglione \textit{et al.} \cite{tartaglione:sensitivity} in which the parameters are pruned using evaluating their sensitivity, defined as the variation of the network output with respect to the parameter.

Due to the scale and the resources required to train and deploy modern deep neural networks, sparse architectures and compression techniques have gained much interest in the deep learning community. Several successful approaches to this problem have been proposed \cite{lebedev:brain_damage, liu:sparse_cnn, zhu:pruning, wen:struct_spars}.
While a more in depth analysis on the topic has been published by Gale~\textit{et~al}.~\cite{gale:state}, in the remainder of this section we provide a summary of the main techniques and their drawbacks.

Multi-objective sparse feature learning has been proposed by Gong~\emph{et~al.}~\cite{gong2015multiobjective}: with their evolutionary algorithm, they were able to find a good compromise between sparsity and learning error, at the cost of high computational cost. 

In their seminal paper~\cite{lecun1990optimal}, Lecun~\textit{et~al.} proposed to remove unimportant weights from a network, measuring the importance of each single weight as the increment on the train error when the weight is set to zero. Unfortunately, the complexity of such method would becomes computationally unbearable in the case of deep topologies with millions of parameters.

\added{Louizos~\textit{et~al.} propose an $\ell_0$ regularization to prune the network parameters during training~\cite{louizos:sparse_l0}. Such a technique penalizes non-zero value of a parameter vector, promoting sparse solutions. As a drawback, it requires solving a complex optimization problem, besides the loss minimization strategy and other regularization terms, using a parameters gating approach through the hard concrete distribution for the parameters.}

\added{Dropout aims at preventing a network from over-fitting by randomly dropping some neurons at learning time~\cite{srivastava:dropout}. Despite the different problem dropout tackles, a number of dropout-inspired techniques aiming at sparsifying deep architectures have been proposed}. Kingma~\textit{et al.}~\cite{kingma:var_dropout} have shown that dropout can be seen as a special case of Bayesian regularization. Furthermore, they use a variational method that allows to use dropout rates adaptively to to the data. Molchanov~\textit{et~al.}~\cite{molchanov:var_dropout} propose Variational Dropout to sparsify both fully-connected and convolutional layers. In particular, the parameters having high dropout rate are always ignored and they can be removed from the network. Even if this technique obtains good performance, it is quite complex and it is reported to behave inconsistently when applied to deep architectures~\cite{gale:state}. Furthermore, this technique relies on the belief that the Bernoulli probability distribution (to be used with the dropout) is a good variational approximation for the posterior.
\added{Recently, knowledge distillation~\cite{hinton2015distilling} received significant attention. 
The goal in this case is to train a single network to have the same behavior (in terms of outputs under certain inputs) as an ensemble of models, reducing the overall computational complexity.
%In order to improve the performance of a deep network, an ensemble of networks is trained and then the average prediction is taken. Recently, it has been observed that the prediction coming from a networks ensemble can be learned by a single network with almost no performance loss. However,
Distillation finds application in reducing the prediction of multiple networks into one, but can not be applied to minimize the computation of the number of neurons for a single network. In general, in distillation-based techniques, the architecture to be trained is a-priori known, and kept static through all the learning process: in this work, we aim at providing an algorithm which automatically shrinks the deep model's size with minimal overhead introduced.} %Such a technique solves a different problem than SeReNe, since in our work we aim at removing single neurons from a model rather than reducing an ensemble of models to just one model.

%AF: qui desriviamo metodsi simili al nostro tipo HAN
Another approach relies on defining the importance of each connection and later remove parameters deemed unnecessary. 
\added{A recent work by Frankle~and~Carbin~\cite{frankle2018lottery} proposed the \emph{lottery ticket hypothesis}, which is having a large impact on the research community. They claim that from an ANN, early in the training, it is possible to extract a sparse sub-network, using a one-shot or iterative fashion: such sparse network, when re-trained, can match the accuracy of the original model. This technique has multiple requirements, like having the history of the training process in order to detect the ``lottery winning parameters'', and it is not able to self-tune an automatic thresholding mechanism.}\\




Han~\textit{et~al.} propose a multi-step process in which the least relevant parameters are defined, minimizing a target loss function~\cite{han:deep_compression}. In particular, it relies on a thresholding heuristics, where all the less important connections are pruned.
In~\cite{tartaglione:sensitivity}, a similar approach was followed, introducing a novel regularization term that measures the ``sensitivity'' of the output wrt. the variation of the parameters. While this technique achieves top-notch sparsity even in deep convolutional architectures, such sparsity is not structured, i.e. the resulting topology includes large numbers of neurons with at least one non-zero parameter. Such unstructured sparsity bloats the practically attainable network footprint and leads to irregular memory accesses, jeopardizing execution speedups.

In this work we aim at overcoming the above limitations proposing a regularization method that produces a \emph{structured} sparsification, focusing on removing entire neurons instead of single parameters.
%In order to achieve this, we compute the sensitivity of the output to the \emph{post-synaptic potential} 
We also leverage our recent research showing that post-synaptic potential regularization is able to boost generalization over other regularizers~\cite{tartaperlo}. 

%\textbf{XXX AF: La ~\cite{cai2017neuralpower} spostata qui dall'intro, da coloocare bene nella sezione}
%As an example, despite the effectiveness of DNNs in solving complex tasks like ImageNet, their deployment on portable or embedded devices has become a growing issue~\cite{cai2017neuralpower}.

==> 4_training_old.tex <==
\section{Pruning Procedure}
\label{sec:training}

This section introduces an iterative procedure to prune a neural network leveraging the sensitivity-based regularization term introduced in the previous section.
We consider some \emph{network model} $M$ that has been preliminary trained at some task over the training set $D$ achieving a satisfying performance level, i.e. greater than $A$ over a validation set $V$.
We do not put any constraint over the actual training method, training set or network architecture, provided that the network can be represented as a-cyclic graph.
In a nutshell, a complete iteration of the procedure consists in the two following steps:

\begin{enumerate}
    \item \emph{Regularization}: we continue training $M$ over $D$ using the update rule \eqref{eq:updaterule} based on our sensitivity-based regularization term. That is, we push towards zero the parameters of neurons with low sensitivity.
    %and validating the model using a randomly-extracted validation set $V$ from the full training set $D$.
    %This means that just the data in $D$, but not in $V$, will be used for the training (and we say, they are grouped in $U$)
    Once a plateau in the performance $A$ is reached, we move to the next stage.

    \item \emph{Thresholding}: parameters lower than a threshold $T$ are set to zero to prune neurons; the threshold value $T$ is maximized while minimizing performance impairment as discussed in Sec.~\ref{sec:Threshold}.
\end{enumerate}

Alg.~\ref{code:serene} summarizes the procedure with pseudo-code. We split the dataset $D$ into disjoint subsets: subset $V$ that is used for validation purpose, and subset $U$ to update the network model.
At line 4 in Alg.~\ref{code:serene} $M$ is first regularized  using the procedure described in details at lines 10-19. 
%, whereas Alg.~\ref{code:finetune} and Alg.~\ref{code:binary} detail the two iterative steps.
Here we promote a sparse model $S$ by training on $U$ according to \eqref{eq:updaterule}.
After every training epoch $S$ is validated on $V$: if the loss value is lower than the previously registered as best model $S_b$, then $S$ becomes the new best. If such an update will not happen for $\textrm{PWE}$ epochs (we call it \emph{plateau waiting epochs}) we assume we reached a plateau and the regularization procedure will return $S_b$.
After the first regularization step we enter the main loop (line 5-9) where thresholding (line 7) and further regularization (line 9) are applied iteratively until the  sparsified model performance is greater than $A$.    

\begin{algorithm}
    \caption{The SE-RE-NE procedure}\label{code:serene}
    \hspace*{20pt}\textbf{Input: }\textit{trained model M, dataset D,\\\hspace*{20pt}Target performance A, PWE, TWT\\}
    \hspace*{20pt}\textbf{Output: }\textit{Final sparsified model S}
    \begin{algorithmic}[1]
        \Procedure{SE-RE-NE}{$M, D, A, PWE, TWT$}
        \State $S_2 \gets M$
        \State $U, V \gets \textsc{RandomSplit}(D)$
        \State $S_2 \gets \textsc{Regularization}(S_2, U, V, PWE)$
        \While {$\textsc{Performance}(S_2, V) > A$}
            \State $S \gets S_2$
            \State $S_2 \gets \textsc{Thresholding}(S_2, V, TWT)$
            \State $U, V \gets \textsc{RandomSplit}(D)$
            \State $S_2 \gets \textsc{Regularization}(S_2, U, V, PWE)$
        \EndWhile
        \Return{$S$}
        \EndProcedure
        \Procedure{Regularization}{$S, U, V, PWE$}
        \State $S_{best} \gets S$\Comment{$S_{best}$ is the best model on $V$}
        \State $epochs \gets 0$
        \While {$epochs < PWE$}
            \State $S \gets \textsc{Train}(S, U)$\Comment{1 epoch on $U$}
            \If{$\textsc{Loss}(S,V) < \textsc{Loss}(S_{best},V)$}
                \State{$S_{best} \gets S$}
                \State $epochs \gets 0$
            \Else{}
                \State $epochs \gets epochs + 1$
            \EndIf
        \EndWhile
        \Return{$S_{best}$}
        \EndProcedure
    \end{algorithmic}
\end{algorithm}


\subsection{Thresholding}
\label{sec:Threshold}
The \emph{thresholding} step follows the regularization step, where parameters of neurons with low sensitivity have been pushed towards zero.
During the threshold stage, parameters whose absolute value is below a given threshold $T$ are pruned away: 

\begin{equation}
    w_{n,i,j} = \left \{ 
    \begin{array}{ll}
       w_{n,i,j} & \left | w_{n,i,j} \right | > T\\
       0    & otherwise
    \end{array}
    \right .
\end{equation}

In order to find a suitable pruning threshold $T$, we look for the $T$ such that the performance (or, in other words, the loss on $V$) worsens at most of a relative value we call \emph{thresholding worsening tolerance} ($TWT$) we provide as hyper-parameter.\\

We expect the loss function to be locally a smooth, monotone function of $T$, for small values of $T$.
%\textbf{ET: forse potremmo specificare QUANTO piccolo deve essere T? O magari si capisce? AF: in effetti non si capisce come scegliere T: se potessimo dare un euristica per trovare un T iniziale da cui partire sarebbe ottimo.ET: in realta' e' spiegato giusto sopra che e' una misura relativa del TWT}\\%A typical observed scenario is shown in Fig.~\ref{fig:lossvserr}.\\
The threshold $T$ can be found using linear search-based heuristics. We can however reduce this using a bisection approach, converging to the optimal $T$ value in log-time steps. %It can be noted that we can effectively use such an approach as the loss function, in the considered cases, is a continuous smooth function.
%The complete procedure is detailed in pseudo-code as Alg.~\ref{code:binary}.


\subsection{Pruned parameter pinning}
\label{sec:finetuning}
%We have observed that iterating regularization and thresholding may significantly impact on converge toward a compressed model.\attilio{Cosa vuol dire la frase precedente ? Che il numero di iterazioni totale e importante o altro ? Se non é fndamentale la toglierei lasciando solo "We have observed that" unendolo alla frase dopo}
In the previous section we have provided an heuristic approach to find the threshold value to prune parameters by the ANN model. However, because of the stochasticity introduced by mini-batch based optimizers, pruned parameters in one thresholding step may be reintroduced by the following regularization steps. %This effect, while from one hand makes the overall sparsification process robust to such a stochastic noise, significantly slows it. 
In order to overcome this effect, we have enforced the constraint that pruned parameters can no longer be updated during the regularization (we term this behavior as \emph{parameter pinning});
%once we prune a parameter (or a whole neuron for instance), we are keeping memory of this and we never again allow it to be reinserted during the regularization step; we call this approach \emph{parameter pinning}. 
to this end, the update rule \eqref{eq:updaterule} is modified as follows:
%\textbf{XXX AF: Dobbiamo trovare un nome per questa cosa che blocchiamo i paramtri a zero: la chiamerei \textit{parameter pinning} ---ET: agreed}
\begin{equation}
    w_{n,i,j}^{t+1} = \left\{ 
    \begin{array}{ll}
        w_{n,i,j}^{t} - \eta \frac{\partial L}{w_{n,i,j}^{t}} - \lambda w_{n,i,j}^{t} \overline{S}_{n, i} & w_{n,i,j}^{t} \neq 0\\
        0 & w_{n,i,j}^{t} = 0
    \end{array}
    \right .
    \label{eq:updatewmem}
\end{equation}
\noindent
%Fig.~\ref{fig:theimportanceofgraveyard} we shows a typical behavior of the compression ratio we achieve as a function of the regularization epochs (with and without parameter pinning). \textbf{XXX AF: Per quae rete in particolare ? La stessa del precedente esempio ? Nota che la compression ratio non l abbiamo ancora definita. Un altro problema e che non e chiaro che meccanismo usiamo per prunare i parametri. Stiamo usando il meccanismo proposto nella sezione successiva ? In tal caso abbiamo un problema logico perche descriviamo la performance di un meccanismo senza aver descritto il meccanismo stesso.}
%It is intuitive that, 
We have noticed that without parameter pinning, the compression of the network may remain low because the noisy gradient estimates in a mini-batch that keep reintroducing previously pruned  parameters.
On the contrary, by adding \eqref{eq:updatewmem} a lower number of epochs are sufficient to achieve much higher compression. 
%After every training epoch on $U$, the model is validated on $V$: if the loss value is lower than the previously registered as best model $S_b$, then $S$ becomes the new best. If such an update will not happen for $PWE$ epochs (we call it \emph{plateau waiting epochs}), we stop our regularization routine, returning $S_b$.
%\textbf{XXX AF Cosa sarebbe un plateau waiting epoch ? Del tipo \textit{se la loss non scende per X epoche} ? ---ET:si}
%The general algorithm is shown in Algorithm~\ref{code:finetune}.
%\begin{algorithm}
%    \caption{Regularization}\label{code:finetune}
%    \hspace*{20pt}\textbf{Input: }\textit{model $S$, training set $U$, validation set $V$, \\\hspace*{20pt}plateau waiting epochs $PWE$}\\
%    \hspace*{20pt}\textbf{Output: }\textit{best model $S_b$}
%    \begin{algorithmic}[1]
%        \Procedure{Regularization}{$S, U, V, PWE$}
%        \State $S_b \gets S$\Comment{$S_b$ is the best model on $V$}
%        \State $e \gets 0$
%        \While {$e < PWE$}
%            \State $S \gets \textsc{Train}(S, U)$\Comment{1 epoch on $U$}
%            \If{$\textsc{Loss}(S,V) < \textsc{Loss}(S_b,V)$}
%                \State{$S_b \gets S$}
%                \State $e \gets 0$
%            \Else{}
%                \State $e \gets e+1$
%            \EndIf
%        \EndWhile
%        \Return{$S_b$}
%        \EndProcedure
%    \end{algorithmic}
%\end{algorithm}


%\textbf{XXX AF in chiusura di questa subsection dobbiamo dire che anche se noi qui pruniamo i pesi indipendentemente, poi sperimentalmente dimostreremo che alla fine andremo a rimuovere interi neuroni}

%With this algorithm we look for the highest $T$ value, say $T^*$, such that the performance of the neural network (i.e. error or loss), doesn't rise above a given upper bound $B$. With this procedure we ensure that the highest number of parameters are pruned away while the performance is still high.

%Following there is the pseudocodes to find the best threshold (Algorithm~\ref{code:binary})  and the relative pseudocodes utilised to do the thresholding (Algorithm~\ref{code:thresh}) and compute the baseline (Algorithm~\ref{code:base}). 

%\begin{algorithm}
%    \caption{Best thresholded model}\label{code:binary}
%    \hspace*{20pt}\textbf{Input: }\textit{model M, validation set V, TWT}\\
%    \hspace*{20pt}\textbf{Output: }\textit{thresholded model S}
%    \begin{algorithmic}[1]
%        \Procedure{Thresholding}{$M,V,TWT$}
%            \State $L_{max} \gets \textsc{Loss}(M, V)\cdot(1+TWT)$
%            \State $a \gets \min_{n,i,j}\{\left | w_{n,i,j} \right |\} $% \Comment $w \in M$
%            \State $b\gets  a\cdot C$
%            \While {$\textsc{Loss}[\textsc{Prune}(M, b)] < L_{max}$} %\Comment{Research of $[a,b]$ range}
%                \State $a \gets b$
%                \State $b\gets a \cdot C$
%            \EndWhile
%            \While {$b-a  > \epsilon$} % \Comment{Research of $T^*$ in $[a,b]$}
%                \State $c \gets (a+b)/2$% \Comment{Midpoint computation}
%                \If{$\textsc{Loss}[\textsc{Prune}(M, c)] < L_{max}$}
%                    \State{$a \gets c$} %\Comment{The new range in which to search $T^*$ is $[c,b]$}
%                \Else{}
%                    \State{$b \gets c$} %\Comment{The new range in which to search $T^*$ is $[a,c]$}
%                \EndIf
%            \EndWhile
%            \State $S \gets \textsc{Prune}(M, a)$
%            \State \Return $S$
%        \EndProcedure
%        
%        \Procedure{Prune}{$M, T$}
%            \ForEach{$w_{n,i,j} \in M$}
%                \If{$\left | w_{n,i,j} \right | < T$} %\Comment{The parameters smaller than $T$ are set to zero}
%                \State{$w_{n,i,j} \gets 0$}
%                \EndIf
%            \EndFor
%            \Return{$M$}
%        \EndProcedure
%    \end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%\caption{Thresholding}\label{code:thresh}
%\hspace*{20pt}\textbf{Input: }\textit{model M, threshold T}\\
%\hspace*{20pt}\textbf{Output: }\textit{thresholded model}
%\begin{algorithmic}[1]
%\Procedure{Thresholding}{$M,T$}
%\ForEach{$w \in M$}
%    \If{$\left | w \right | < T$} %\Comment{The parameters smaller than $T$ are set to zero}
%        \State{$w=0$}
%    \EndIf
%\EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

%\begin{algorithm}
%\caption{Compute baseline}\label{code:base}
%\hspace*{20pt}\textbf{Input: }\textit{model M, dataset D, labels L}\\
%\hspace*{20pt}\textbf{Output: }\textit{baseline $\beta$}
%\begin{algorithmic}[1]
%\Procedure{ComputeBaseline}{$M,D, L$}
%\State{$output \gets M(D)$} \Comment{Model is applied to the dataset}
%\State{$ \beta \gets \textsc{Criterion}(output, L)$} \Comment{Loss or error is computed comparing the %output to the labels}
%\State \Return $\beta$
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

%The algorithm is simple, but deserves some explanations. First of all we search a range $[a,b]$ in which we search $T^*$. As $a$ we choose the minimum of all parameters in absolute value of the network. As $b$ we choose the first value that causes the decay of the performance $\beta$, after the thresholding with $b$. In particular, we start from $a$ and we multiply it by $C$, until the performance doesn't raise above the upper bound $B$. Once we have found the range $[a,b]$, bisection starts finding $T^*$ having as reference the performance $\beta$. Every after bisection step, model parameters are restored because the monotonicity of $T^*$ is not guaranteed.

%During the training it is possible that already pruned parameters may be reintroduced. This is caused by the gradient $\frac{\partial L}{\partial w_{n,i}}$, associated to the parameter $w_{n,i}$, used in the update rule. If said value is big enough to overcome the thresholding step the parameter is reintroduced in the network. Since reinserted parameters may bring the network in a sub-optimal configuration, we introduce the \textit{third step} that doesn't allow the pruned parameters to be restored. This is accomplished by building, before each training step, a binary matrix (\textit{i.e.} a $mask$) that stores which parameters are active and which are already removed. After the update and thresholding steps all parameters are multiplied by the mask, that push to zero the parameters eventually reintroduced.

